MMDT: Decoding the Trustworthiness and Safety of Multimodal Foundation Models

Multimodal foundation models (MMFMs) play a crucial role in various applications, including autonomous driving, healthcare, and virtual assistants. However, several studies have revealed vulnerabilities in these models, such as generating unsafe content by text-to-image models. Existing benchmarks on multimodal models either predominantly assess the helpfulness of these models, or only focus on limited perspectives such as fairness and privacy. In this paper, we present the first unified platform, MMDT (Multimodal DecodingTrust), designed to provide a comprehensive safety and trustworthiness evaluation for MMFMs. Our platform assesses models from multiple perspectives, including safety, hallucination, fairness/bias, privacy, adversarial robustness, and out-of-distribution (OOD) generalization. We have designed various evaluation scenarios and red teaming algorithms under different tasks for each perspective to generate challenging data, forming a high-quality benchmark. We evaluate a range of multimodal models using MMDT, and our findings reveal a series of vulnerabilities and areas for improvement across these perspectives. This work introduces the first comprehensive and unique safety and trustworthiness evaluation platform for MMFMs, paving the way for developing safer and more reliable MMFMs and systems. Our platform and benchmark are available at https://mmdecodingtrust.github.io/.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{All the claims are made by rigorous empirical validations for all trustworthiness perspectives in the paper.}
  \item Did you describe the limitations of your work?
    \answerYes{The limitation is discussed in \Cref{app:limitation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The impact is discussed in \Cref{app:impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We read and ensure that the paper conforms to the ethics review guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{No theoretical analysis is presented in the paper.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{No theoretical analysis is presented in the paper.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All the data, codes, and instructions are provided at \url{https://mmdecodingtrust.github.io/}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All the details are provided in the Appendix as well as the code repo at \url{https://mmdecodingtrust.github.io/}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We control the random seeds and evaluate with multiple times to control the evaluation randomness.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We include all details in Appendix and our benchmark website tutorial \url{https://mmdecodingtrust.github.io/}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite all used assets (e.g., MS COCO dataset).}
  \item Did you mention the license of the assets?
    \answerYes{We mention the license in Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We creat novel benchmark and provide it at \url{https://mmdecodingtrust.github.io/}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We follow the license to use all publicly available data. There is no specific consent from people involved.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We carefully identify the potential privacy leakage and offensive content and discuss the safeguard of such data usage in \Cref{app:impact}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We do not involve any crowdsourcing or human subject research.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We do not involve any crowdsourcing or human subject research.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We do not involve any crowdsourcing or human subject research.}
\end{enumerate}

\end{enumerate}

==> figures/platform.tex <==
\begin{figure}[t]
    \centering
    \small
    \includegraphics[height=1.0\textheight]{figures/platform_pdf.pdf}
    \caption{\small A tree taxonomy of different perspectives of trustworthiness that our benchmark focuses on.}
\label{fig:taxonomy}
    % \vspace{-0.25in}
\end{figure}

==> tables/hallucination/i2t_main.tex <==
\begin{table}[t]
    \centering
    \caption{Accuracy of image-to-text models for hallucination evaluation.}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c|ccccc|c}
    \toprule
         \bf Model & \bf Distraction & \bf Counterfactual & \bf Co-occurrence & \bf Misleading & \bf OCR & \bf Average \\
         \midrule
         {\gptv}  
         & - & - & - & 52.2 & 26.2 & - \\
         {\gpto}  
        & - & - & - & 43.2 & 36.8 & - \\
        {\llava}  
        & - & - & - & 34.2 & 14.4 & - \\
    \bottomrule
    \end{tabular}%
    }
    \label{tab:i2t_main}
\end{table}

==> tables/hallucination/t2i_main.tex <==
\begin{table}[t]
    \centering
    \caption{Accuracy of text-to-image models for hallucination evaluation.}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c|ccccc|c}
    \toprule
         \bf Model & \bf Distraction & \bf Counterfactual & \bf Co-occurrence & \bf Misleading & \bf OCR & \bf Average \\
         \midrule
         % \multirow{4}{*}{\shortstack[l]{llava-hf/\\llava-v1.6-\\mistral-7b}}  
         {\sdxl}  
         & -  & - & - & 30.4 & 20.2 & - \\
         % \multirow{4}{*}{\shortstack[l]{Salesforce/\\instructblip-\\vicuna-7b}}  
         {\dream}  
         & -  & - & - & 32 & 26 & - \\
         {\openjourney}  
         & -  & - & -& 28.4 & 29.6 & - \\
         {\dfif}  
         & -  & - & 31.8 & 30.6 & 12.4 & - \\
         {\dalleII}  
         & -  & - & - & 29.2 & 11.2 & - \\
         {\dalleIII}  
         & -  & - & - & 45.8 & 21.2 & - \\
    \bottomrule
    \end{tabular}%
    }
    \label{≈}
\end{table}

==> tables/ood/t2i_challenge.tex <==
\begin{table}[ht]
\caption{OOD results on text-to-image Challenge Data. The numbers in parentheses represent the original scores of these data. The best scores for each type are bold.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|c|cccc}
\toprule
\textbf{Model} & \textbf{Type} & \textbf{Overall} & \textbf{Usefulness} & \textbf{Counting} & \textbf{Spatial} & \textbf{Attributes}\\\midrule
%  \multirow{2}{*}{sd2.1}  & Shake & 20.68 (56.09) & 60.72 (85.38)  &  12.00 (62.00) & 4.00  (28.00) & 6.00 (49.00) \\
% & Rare Ling.  & 25.87 (54.20) & 68.47 (85.78) & 20.00 (61.00) & 2.00 (23.00) & 13.00 (47.00) \\\midrule
%  \multirow{2}{*}{kandinsky-3}  & Shake & 38.02 (64.59) & 74.07 (89.35)  &  47.00 (70.00) & 11.00  (45.00) & 20.00 (54.00) \\
% & Rare Ling.  & 36.58 (64.12) & 78.31 (88.48) & 34.00 (71.00) & 13.00 (38.00) & 21.00 (59.00) \\\midrule
%  \multirow{2}{*}{OpenDalleV1.1}  & Shake & 31.46 (72.64) & 73.86 (95.58)  &  36.00 (68.00) & 7.00  (69.00) & 9.00 (58.00) \\
% & Rare Ling.  & 35.69 (76.77) & 79.77 (94.09) & 30.00 (70.00) & 15.00 (76.00) & 18.00 (67.00) \\\midrule
 \multirow{2}{*}{stable-diffusion-xl-base-1.0}  & Shake & 26.96 (53.56) & 68.84 (89.24)  &  23.00 (47.00) & 8.00  (43.00) & 8.00 (35.00) \\
& Rare Ling.  & 34.93 (54.14) & 74.74 (88.56) & 30.00 (47.00) & 11.00 (40.00) & 24.00 (41.00) \\\midrule
 \multirow{2}{*}{openjourney-v4}  & Shake & 29.67 (43.24) & 70.67 (85.98)  &  28.00 (41.00) & 8.00  (24.00) & 12.00 (22.00) \\
& Rare Ling.  & 34.10 (41.01) & 76.39 (85.03) & 35.00 (37.00) & 10.00 (15.00) & 15.00 (27.00) \\\midrule
 \multirow{2}{*}{dreamlike-photoreal-2.0}  & Shake & 29.77 (44.22) & 68.08 (87.86)  &  33.00 (41.00) & 7.00  (20.00) & 11.00 (28.00) \\
& Rare Ling.  & 33.08 (41.44) & 76.33 (86.77) & 34.00 (39.00) & 7.00 (13.00) & 15.00 (27.00) \\\midrule
 \multirow{2}{*}{DALL-E 2}  & Shake & 30.86 (54.39) & 65.42 (85.57)  &  44.00 (64.00) & 6.00  (28.00) & 8.00 (40.00) \\
& Rare Ling.  & 36.46 (55.06) & 72.83 (85.23) & 45.00 (63.00) & 8.00 (31.00) & 20.00 (41.00) \\\midrule
 \multirow{2}{*}{DALL-E 3}  & Shake & 54.63 (72.73) & 76.51 (86.93)  &  57.00 (60.00) & 26.00  (63.00) & 59.00 (81.00) \\
& Rare Ling.  & 57.53 (72.19) & 77.13 (85.77) & 58.00 (58.00) & 41.00 (63.00) & 54.00 (82.00) \\ \bottomrule
\end{tabular}
}
\label{tab:ood_t2i_challenge}
\end{table}
